Bugs in our Pockets: The Risks of Client-Side Scanning

Our increasing reliance on digital technology for personal, economic, and government affairs has made it essential to secure the communications and devices of private citizens, businesses, and governments. This has led to pervasive use of cryptography across society. Despite its evident advantages, law enforcement and national security agencies have argued that the spread of cryptography has hindered access to evidence and intelligence. Some in industry and government now advocate a new technology to access targeted data: client-side scanning (CSS). Instead of weakening encryption or providing law enforcement with backdoor keys to decrypt communications, CSS would enable on-device analysis of data in the clear. If targeted information were detected, its existence and, potentially, its source, would be revealed to the agencies; otherwise, little or no information would leave the client device. Its proponents claim that CSS is a solution to the encryption versus public safety debate: it offers privacy -- in the sense of unimpeded end-to-end encryption -- and the ability to successfully investigate serious crime. In this report, we argue that CSS neither guarantees efficacious crime prevention nor prevents surveillance. Indeed, the effect is the opposite. CSS by its nature creates serious security and privacy risks for all society while the assistance it can provide for law enforcement is at best problematic. There are multiple ways in which client-side scanning can fail, can be evaded, and can be abused.

==> dregs.tex <==



%\documentclass{article}
%\usepackage{footmisc}
%\usepackage[utf8]{inputenc}

%
% Use this line for law-style footnotes (and, if we wish, delete the \printbibliography at the end)
%
\usepackage[notes,strict,backend=biber,autolang=other,bibencoding=latin1,related=true,idemtracker=constrict]{biblatex-chicago}

%
% Use this for traditional tech-style bibliographies 
% https://www.overleaf.com/project/607104386e78ae7c2cd1d648
%
%\usepackage[backend=biber,autolang=other,bibencoding=latin1,related=true,idemtracker=constrict]{biblatex}

\usepackage[pdftex,colorlinks,allcolors=blue]{hyperref}
%https://www.overleaf.com/project/607104386e78ae7c2cd1d648
\bibliography{key-risks}

\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Section}
\renewcommand{\figureautorefname}{Figure}

\title{Bugs in our Pockets:\\The Risks of Client-Side Scanning}
\author{
Hal Abelson\thanks{Massachusetts Institute of Technology.} \and
Ross Anderson\thanks{Cambridge and Edinburgh Universities.} \and
Steven M. Bellovin\thanks{Columbia University.} \and
Josh Benaloh\thanks{Microsoft Research.} \and
Matt Blaze \and
Whitfield Diffie \thanks {Chief Security Office, Sun Microsystems Retired} \and
John Gilmore\thanks{The Electronic Frontier Foundation.} \and
Matt Green \and
Susan Landau\thanks{The Fletcher School and School of Engineering, Tufts University.} \and
Peter G. Neumann\thanks{SRI International Computer Science Lab.} \and
Ronald L. Rivest\thanks{Massachusetts Institute of Technology.} \and
Jeffrey I. Schiller\thanks{Massachusetts Institute of Technology.} \and
Bruce Schneier\thanks{Harvard Kennedy School.} \and
Michael A. Specter\thanks{Massachusetts Institute of Technology.}  \and
Vanessa Teague\thanks{Thinking Cybersecurity Pty. Ltd. and the Australian National University.}  \and
Carmela Troncoso\thanks{Ecole Polytechnique Federale de Lausanne.} \and
Danny Weitzner
}
\date{rev. \today}

\begin{document}

\maketitle

\section*{Executive Summary}
% https://www.overleaf.com/project/607104386e78ae7c2cd1d648
Public access to strong cryptography has been contentious since the mid-1970s. National-security forces tried to limit its use, then law-enforcement agencies subsequently pressed to do so. 
Numerous proposals have been suggested, including key-escrow and `exceptional access' mechanisms; none have found wide acceptance. Now some in industry and 
government are advocating ``client-side scanning'' as a silver-bullet solution to their encryption quandary. 

Client-side scanning is hailed as a `perfect' solution that would enable monitoring, while leaving security and privacy intact. Instead of weakening encryption or providing law enforcement with back-door keys, client-side scanning would enable on-device analysis of data \emph{in the clear}. If targeted information were detected, its existence, and potentially its source, would be revealed to the enforcement bodies. Otherwise, we are assured that the use of client-side scanning would neither weaken nor prevent the use of end-to-end encrypted communications.

However, such scanning is not without significant technical and operational issues:
\begin{itemize}
\item Automated scanning is already in use privately by cloud and social-media providers. It frequently generates false-positive signals (the declaration that something inappropriate is happening, when in fact it is not).

\item The signals from scanning systems are often considered to be authoritative, requiring flagged individuals to prove their innocence---often after sanctions have already been applied. In the case of government-sponsored client-side scanning, such sanctions may result in loss of freedom, instead of just inconvenience.
\end{itemize}

Of even greater concern is the introduction of significant security risks to an already fragile communication and computation infrastructure. Any deployed technology has the potential to be circumvented or reused by bad actors. For instance, the first time client-side scanning was deployed at scale was the Chinese `Green Dam' filter in 2009; perhaps inadvertently, this enabled any website a user visited to take control of their PC.
To accommodate changing law-enforcement requirements, the rules that identify targeted content can be arbitrarily complex, may change over time, and must often be kept secret (which is impractical on insecure consumer devices). 


The main advantage of CSS---that it can be done privately, on the client device---is a cause of its main weaknesses. Due to the insecurity of user devices, the surveillance and control capabilities provided by CSS cannot be owned by those deploying it, but are potentially available to any adversary. This includes criminals and enemy nations that can compromise the device or any entity in the chain that sets or updates the scanning policy. Resisting attempts to spy and influence non-criminal citizens is possibly the highest priority of our national security, but client-side scanning does exactly the opposite. 
The security of client-side scanning is made worse by the opacity of mobile operating systems, which hinders any attempt to ensure that policies are updated only by legitimate actors. 

The risks associated with client-side scanning may extend to all of society, not just to criminal suspects. In particular, when it is not limited to targeted devices, but installed on everyone's, it threatens the security of lawbreakers and law-abiding citizens alike. Client-side scanning gives government agencies access to content, and so must be treated like wiretapping; in jurisdictions where bulk intercept is prohibited, bulk client-side scanning must be as well.


Its proponents claim that client-side scanning allows end-to-end encryption, but this is only after the communication has already been scanned for targeted content. Therefore, it is still bulk intercept, just automated and distributed. The ability of citizens to communicate freely depends strongly on their ability to feel safe in doing so.  Such surveillance carries with it many dangers, including the fact that those in the middle of the political spectrum would be most intimidated from participating in the political process.  In these times of sharp polarization, silencing the center creates real dangers. The specter of `Big Brother' can provide a significant chilling effect on freedom of speech and, indeed, on democracy itself.

\section{Introduction}

As modern cryptography has become available to the public, the technology has become mired in conflict. Companies and individual citizens---and even governments---need online security and privacy, both of which depend on cryptography in complex ways. 

Over the past forty years, the agencies' playbook has evolved from trying to limit the use of strong cryptography, through demanding access to civilians' cryptographic keys, to obtaining access to stored versions of encrypted communications via services such as Gmail and Facebook. 

Yet, there are tensions both within and between governments. Twenty years ago, the European Union and the U.S. loosened export controls on products with strong encryption. Since that time, U.S. law enforcement has repeatedly demanded controls on encryption, while its national-security leaders have largely been silent on the issue. %By contrast, both European Union law-enforcement and national-security agencies have sought controls. 
For a time, the stated concern was terrorism; of late, the narrative in both Europe and the U.S. has been about child sex-abuse material (CSAM)~\autocite{DOB-eff2020}. 
India also seeks to restrict the use of strong encryption tools, to trace people who oppose  the government's policies~\autocite{BBC-india2021}. 
Recent legislation in Australia similarly seeks to force government access to encrypted communications\autocite{Aus_TOLA}. 
Overall, many law-enforcement and some national-security agencies claim that the availability of cryptography threatens their ability to carry out their missions\autocite{Wray2021, FCM}. 

The latest evolution has seen some agencies demanding to scan all communications from phones, laptops, and other devices before they are sent: so-called {\em client-side scanning} (CSS). 
In some cases, agencies want to forward the communication to government investigators or to block sending entirely. 
This capability would be installed on selected apps on all devices of all users, not just those under a court order. 

This raises many of the old objections, and some new ones too. In this paper we analyze the risks and costs of client-side scanning at scale, and show that it is unlikely to provide any silver-bullet solution to public-policy problems. 

\section{Background}

Government demands for access to encrypted data have a long history. In the early years, controls centered around prohibiting export and surreptitiously weakening encryption algorithms and products. 
In the 1990s and 2000s, controls switched to various ``key escrow'' proposals: mechanisms to ensure government access to keys. 
In the 2010s, the focus switched to accessing data on corporate servers and breaking encryption on end-user devices such as smart phones. 
In all cases, these demands for access pitted the demand for surveillance against the security of encrypted communications. 
Many of the authors of this report participated in these debates, and wrote two reports analyzing the security of government proposals: first in 1997 and again in 2015\autocite{1997Report,KUD}.\footnote{An expanded history of the `Crypto Wars', as they are colloquially known, is included as Appendix I.} As researchers who work at the intersection of technology and policy, our goal here is to examine the security implications of governments enforcing policy by mandating the installation of surveillance and control mechanisms in end-user devices such as phones and laptops.

Many changes have occurred since 2015, including:

\begin{itemize}
    \item Increasingly serious cyberattacks against public and private networks, with many governments and even criminal enterprises now having the capability to cause grave harm (Solarwinds, Kaseya);
    \item Such attacks have even been made against critical infrastructure (attacks on the Ukraine electricity grid and the Colonial Pipeline);
    \item Easier access to invasive tools, ranging from police use of forensic tools that give access to seized devices and the services to which they have access, through the industrial-scale compromise of user devices by organized crime groups, to the sale of high-end phone surveillance systems such as NSO's Pegasus to authoritarian governments;
    This is the longest nonsentence I have seen in a long time---there is no MAIN VERB, as in the previous item.  All of these items should be parallel constructs.  With a verb or two this one could be split up into multiple senences. But then the other three items should be made into grammatical sentences.  Alternatively, the second item should not be a grammatical sentence.  End of PGN-rant
    \item Greater use of encryption by the public, including over a billion users of WhatsApp---which employs end-to-end encryption---and the proposal from Facebook to extend this to Facebook Messenger;
    \item The spread of communication platforms such as TikTok that are based and controlled in China, reversing the privileged global access previously enjoyed by the NSA.
\end{itemize}

There have increasing concerns by some governments regarding certain types of crime (e.g., CSAM). The demand in July 2020 by the German Presidency of the EU that end-to-end encrypted messaging services such as WhatsApp have an `upload filter' to enable the authorities to scan for illegal content has raised the prospect of a rerun of the Crypto Wars~\autocite{DOB-eff2020}. 
The idea is that every smart phone and computer would have software, controlled by a third party, that would monitor the user and alert someone if the user performed any one of a variety of targeted actions---for example, sending illegal material to another user. 
This approach would circumvent encryption by monitoring the content prior to the user encrypting and sending it.
The intent is the same---government access to encrypted data---but the architecture would enable access to client devices through surveillance software run on those devices. 
This was supported in October 2020 by a joint statement by the justice ministers of the Five Eyes countries  calling on technology companies to help find ways to ensure that those committing serious crimes such terrorism and child sexual abuse were not protected by end-to-end encryption~\autocite{PBDLB2021}. This was also co-signed by India and Japan but ministerial names were not supplied.



While the conflicts of the 1970s to the 1990s centered on security versus privacy, the issue is no longer just privacy versus security;
%a conflict over efficiency of law-enforcement investigations versus the security of individuals, firms, and states. The policy debate is less a `war' between two sides, and more a question of balancing different security needs. Or 
as the 2019 Carnegie Endowment for International Peace study on cryptography policy observed, ``Security in the context of the encryption debate consists of multiple aspects including national security, public safety, individual cybersecurity and privacy, and security from hostile or oppressive state actors.''\autocite{CEIP2019}\footnote{Members of the study included Jim Baker, former General Counsel, FBI; Tom Donahue, former Senior Director for Cyber Operations, National Security Council; Avril Haines, former Deputy Director, CIA, former Deputy National Security Advisor, and current Director of National Intelligence; Chris Inglis, former Deputy Director, NSA; Jason Matheny, former Director, IARPA; Lisa Monaco, former Assistant to the President for Homeland Security and Counterterrorism; as well as two members of this group, Susan Landau and Ronald Rivest.} We build on the Carnegie work, using the principles developed there to guide our recommendations on client-side scanning. 
and on the 2018 U.S. National Academies of Science, Engineering, and Medicine  encryption study~\autocite{NASEM2018}


%Many issues in the encryption controversies hinge on how policy and technology interact. 
%As researchers who work at this intersection, we have contributions to make. 
%Our goal here is to examine the security implications of governments enforcing policy by mandating the installation of surveillance and control mechanisms in end-user devices such as phones and laptops. 
This includes the bulk recording of information for later enforcement action, the direct limitation of some activities, and actions to target some subset of users.  

Different governments target different information. 
In focusing on the technical issues, we are deliberately not distinguishing between those forms of information that we find universally offensive (e.g., terrorist advocacy) from those that are prohibited in some countries (e.g., pro-democracy advocacy)
For brevity's sake we refer to the mechanisms used to select, collect and block targeted information simply as `control mechanisms'.

\section{Content Scanning Technologies}

Many online service providers perform automated scanning to detect illegal content, such as sexual-abuse material and terrorist-recruitment videos. 
Historically, these scanning mechanisms have been implemented within provider-operated servers. 

\subsection{Scanning on the Server Side}


Depending on the type of content, positive matches can be flagged for manual review by human beings, or reported to law-enforcement agencies for further action.\footnote{In the U.S.A., providers are legally required to manually examine flagged CSAM content, and then submit reports to a clearinghouse operated by National Center for Missing and Exploited Children.}
At least two different technologies are currently used to implement content scanning: various types of hashes and machine-learning techniques. 

For CSAM, the most common technique compares user files with a list of hashes of known illicit images, which is assembled by providers or by organizations such as the National Center for Missing and Exploited Children (NCMEC). 
Hashing is a way of compressing data that provides a `signature'; a refinement of the technique uses `perceptual hashes'.
Perceptual hashing is designed so that a small change in the input (such as a slight change of the position of a curtain in a photo) results in only minimal change of the hash. 
This supports inexact matches: providers can detect known content even when it has been slightly modified (\textit{e.g.,} rotated, cropped, or re-encoded as a new image file.) 
Again, providers match user files against a list of hashes using perceptual-hashing algorithms such as Microsoft's PhotoDNA and Facebook's PDQ~\autocite{photodna,Newton2019Facebook-open-s}.

A newer, more experimental, approach uses machine-learning (ML) techniques to identify targeted content. 
The provider first trains a machine-learning model over a training set comprising known illegal images. 
This model is then used to identify illegal images uploaded by users. 
It is claimed to be able to detect previously unrecognized illicit content, potentially at the cost of a higher error rate.
However, experiments have shown that even imperceptible changes to an image can cause misidentification~\autocite{Goodfellow2015Explaining-and-}, as we explain later. 

While these two scanning technologies operate differently, they share some common properties. Both require the user to submit unencrypted content for matching by the provider; both can detect files that the system has not seen before, though at the cost of a non-zero false positive rate. Finally, both methods rely on a proprietary tool (a model or a hash list) developed from a corpus of known illegal content. Some scanning techniques also use proprietary algorithms. For example, the technology behind Microsoft's PhotoDNA is available only  to partner organizations under a non-disclosure agreement.

Regardless of the underlying technique, each of these techniques can be treated as a black box that takes in user images, and outputs a determination of whether one of them matches. 
The scanning system therefore requires access to cleartext (i.e., unencrypted) user files in order to scan them. 


\subsection{Scanning in End-to-End Encrypted Systems} 
\label{sec:scanningin}

Historically, service providers have implemented scanning within a centralized online server, backed up with human reviewers. 
This approach is expensive but has several benefits: the provider can evaluate all user images without needing to publish the algorithms and/or model that is used to detect those that are illegal. 
Normally the model (or hash list) and the scanning algorithms are made available only to partners under a non-disclosure agreement. 
The model may be a trade secret, and the possession of such images is in any case an offense in the absence of a lawful excuse. 
Yet the deployment of end-to-end encrypted communications prevents centralized content scanning, as service providers no longer have access to user plaintext. 
As a side-effect, they save the costs of scanning.

Both policymakers and engineers sometimes fail to understand the scale of modern global messaging systems.
While an organization with 10,000 people might run a single mail server, an email service or chat system that is used by a billion people will have tens of thousands of servers.
And while a spam filtering system designed by an individual researcher for their own use might be claimed to be effective if it stopped 95\% of unwanted messages, a 5\% error rate is intolerable at Internet scale.
Large service firms require very much smaller false-positive rates; 5\% of 10 billion WhatsApp messages a day would mean 500 million false alarms.
This is particularly important when filtering content such as terrorist material of which there is very little.
If only one message in ten million is of relevance to terrorism---the `base rate'---then even if the filter has a false-positive rate of only one in a thousand, there will still be 10,000 false positives for every genuine terrorist message that is found.
To find any of these messages in practice requires secondary filtering, by further automated systems and then by human reviewers, whose costs are substantial.


It is in this context that we must consider the proposal to detect CSAM in end-to-end encrypted systems via client-side scanning. 
Not one of the many ML models works well on this problem. 
First, the ML models currently in use have to be large in order to achieve enough precision; the European Commission's own leaked technical report suggested that the client-side software would have to send many samples to a server for more detailed analysis~\autocite{EU_Tech_Sol_2020}. 
Second, ML models are vulnerable to adversarial samples; an adversary who has access to them, or who can test their responses repeatedly, can learn how to tweak inputs to cause both false negative and false positive errors---that is, that targeted material can slip through while innocuous material is flagged~\autocite{biggio2013evasion,szegedy2013intriguing}.

The same holds for perceptual hashing. 
Recent research demonstrated ways that images can be minimally modified, and yet change the perceptual hash sufficiently so that the image is no longer recognized as targeted content~\autocite{JainCretudeMonteye}. % {\bf Carmela to add more detail, examples, and references here.}

As client-side scanning cannot be sufficiently precise and would generate too many false positives, it is extremely likely that suspect content would be referred to existing server-based scanning systems for secondary examination.
Thus, while its proponents claim that client-side scanning resolves the scanning problem without compromising end-to-end encryption, closer examination demonstrates that user privacy is compromised, and quite possibly without even saving scanning costs. 
In fact, the situation is worse than that; client-side scanning introduces serious security risks, which we describe next.


\section{Attacks on Client-Side Scanning}

Traditional end-to-end encrypted systems provide confidentiality for user communications, even when the service provider is not trusted. Client-side scanning will undo this protection.

As a practical matter, any client-side filters are almost certain to require frequent communication with servers. 
The models used to detect illegal content are likely to be rapidly circumvented if they are published, or if adversaries can probe them with enough test images; the newer machine-learning models have to be large to avoid too high a rate of false positives. 

Just as a smart speaker uses local logic to listen for a `wake word' and then sends user speech to the cloud for processing, so also a client-side filter would contain limited functionality, and refer a large number of slightly suspect images to cloud-based servers for more detailed processing. 
This is also the conclusion of the leaked EU discussion paper~\autocite{EU_Tech_Sol_2020}.
Because of the scale and complexity of the existing scanning operation, suspect material would most likely be referred to the existing server-side filters---which themselves refer millions of suspect messages and photos to human reviewers every hour of every day.  
Thus client-side scanning systems are at best described as providing `selective confidentiality' and require the user to trust the service provider. The design goal of these systems is to ensure that targeted content can be flagged, blocked, or reported, while other user content remains confidential.

 
This two-tier design implies that client-side scanning fundamentally changes the confidentiality guarantees of an end-to-end encrypted system. The security would then instead be dependent on the underlying scanning algorithms, the protocols for dealing with targeted content, the mechanisms for maintaining these protocols, and the back-end surveillance infrastructure in the cloud. Client-side scanning effectively downgrades the end-to-end encryption to be little better than the old-fashioned server-based systems. In effect, while Facebook was talking of making Messenger as secure as WhatsApp by adding end-to-end encryption, the EU proposal would make WhatsApp no more secure than Messenger.

The deployment of client-side scanning raises several new security concerns that are not as salient in provider-side scanning systems:

\begin{description}

\item {\em Model information leakage.} Client-side scanning systems require providers to move at least parts of their sensitive models (or hash lists) out of centralized servers, and to deploy them within client applications. This increases the probability that adversaries, whether users or others, would reverse-engineer the application to extract the model and even extract sensitive illicit information from it. This is particularly concerning for systems based on neural networks. Research has shown that sensitive training inputs can be extracted from these models, and that such attacks are quite difficult to prevent~\autocite{TMWP2020}. Because it would be unacceptable to risk further traumatizing abuse victims by providing abuse imagery to attackers, large parts of the models and hash lists would need to reside in the cloud.


\item {\em False positives.} Content scanners are designed to find approximate matches to illegal files so they can recognize content that has been re-encoded or tweaked. 
ML-based systems are designed to identify entirely new content that is somehow similar to known illegal content. 
In both cases, false positives are certain: some legal content will be flagged as suspect. 
The likelihood of false positives is increased by differences between the distribution of training data and the distribution of the data encountered in the wild. 
This difference, known as {\em distributional shift}, can increase the number of errors. 
More worryingly, this error increase tends to affect particular subsets of samples, typically for minorities. 
The move from centralized to distributed scanning may make fairness harder to monitor.

Even if false positives occur with low probability, existing messaging systems operate at hyperscale: many billions of messages are sent each day. 
If false positives were only one in a thousand, millions of messages would have to be assessed centrally, imposing very high costs on service providers. 


\item {\em Model poisoning.} A more critical concern is that the scanning model (or hash list) could be {\em poisoned}.  
(Poisoning arises when an adversary develops illicit content which, when incorporated into a scanning model, causes the model to either fail to trigger on some class of illicit inputs, or to give a false alarm when exposed to legitimate content.)  
Having poisoned a scanning model, an adversary might monitor the client's network connection for signs of a positive match, or collude with insiders at the provider to detect alarms that targeted specific users. 
Model poisoning can occur even if the provider and model builder behave honestly. 
Preventing poisoning is challenging, while defending against poisoning is a major open research problem for which a solution may not exist.

\item {\em Evasion.} A final concern in client-side systems is the possibility that some users will reverse-engineer them and use the resulting knowledge to evade scanning entirely. 
In the simplest case, people may simply avoid transmitting content that is known to trigger scanning filters. 
Others may alter the client software to disable scanning subroutines. 
More sophisticated adversaries will develop ways to alter content so as to cause errors---whether false negatives (where illicit content is designed to escape surveillance), or false positives (where innocuous content is altered to cause alarms at such a scale as to swamp the defences). 
Given access to models or even to training data, the techniques of adversarial machine learning can be used to develop ways of tweaking images so that they will escape the filter~\autocite{biggio2013evasion,szegedy2013intriguing} or even jam the filter. 

\item {\em Accountability of model / hash list} 
The requirements to protect information leakage conflict with those needed to ensure accountability. 
Existing provider-side scanning systems train on abuse data collected by the provider, or purchased from agencies such as NCMEC; there is little public visibility of this process. 
In client-side scanning systems, scanning using unknown models poses a novel surveillance risk---as any content that is identified by the model may be subject to interception.
When models are not public---and because their training sets are illegal, they cannot be made public---it is extremely difficult to know what content is extracted from peoples' phones. 
The situation is made worse by the fact that since new illegal content arises frequently, models must be updated periodically; this means that surveillance activities must, by design, evolve and broaden without public oversight. 
Even if the intercepted content is encrypted en route to the service provider or law-enforcement agency, local traffic analysis can disclose the fact that a certain device is now subject to interception.

\end{description}

\section{Further Risks Posed by Client-Side Scanning}

Further security risks posed by client-side scanning will depend on where in the client the scanning is done (in one app, in many apps or in the operating system); which governments have access; how the scope and purpose of the scanning is limited by both law and technology; and limits imposed by complexity.

\subsection{The Location of Scanning}

If, as the UK has proposed, the regulator imposes a harm-reduction duty on the service provider, they might be tempted to turn off end-to-end encryption for images and video streams coming from countries that are known sources of illegal content.\footnote{Images are typically kept encrypted on the server until the recipient taps on a thumbnail version of the image to download the full image. The encryption keys are managed centrally when there is more than one recipient. The service provider could simply decide that it is also a recipient of all messages coming from problematic countries, and feed them into its usual filtering mechanisms.}
However the regulator could find many arguments why this might not be sufficient.

If, as the EU has proposed, controls are to be mandated in communications apps with more than a certain number of users, then perhaps WhatsApp would be monitored, while less popular apps such as Signal would continue to provide end-to-end privacy.


Consider what options might be possible for such controls. 
In chat apps, data such as the sender, the receiver, their status, group membership, location, read receipts and much else need to be understood and acted on by the chat server.\footnote{These communications are typically protected by an outer layer of TLS encryption, but can be retrieved by investigators through warrants or, in many cases, by man-in-the-middle attacks.} 
Thus the apps ship most of their metadata outside the `envelope' of the end-to-end encryption, and these metadata are used, for example, by Facebook for ad targeting in WhatsApp.
If such analyses are to be extended to include access to end-to-end encrypted content, then the natural architecture would be for each WhatsApp client to contain a listening post  that communicates with the secondary screening server; if this server were not at Facebook but elsewhere, then metadata would presumably have to be copied too.
The surveillance could be done most efficiently at Facebook, which, as noted above,  already has the many thousands of servers required to do secondary screening of suspicious content.
This would be the preferred route from a security point of view; any other solution, such as police stations around the world, would introduce uncontrollable security risks.  

If the scanner is installed at the level of the operating system, it could monitor other apps and control the device itself. 
The standard operating procedure in targeting a suspect's phone involves taking over an app, and then using a `privilege escalation' vulnerability to install a `remote access Trojan' in the device's operating system. 
This enables investigators to copy all the data from the device, record unlock passwords, and even turn on the microphone and camera silently so that the phone becomes a covert surveillance device.
With full access to the device, investigators can also do `cloud forensics'---which means that they download the cookies used to give access to services such as mail, and download all the suspect's mail to their own servers for examination.
If the scanning code is buggy, it could be exploited remotely to the same effect.

In at least some countries, the government is likely to require that the Listening Post have the following capabilities:

\begin{enumerate}
    \item As a minimum, read access to files stored in the WhatsApp directory---including drafts, sent and received messages, and photos---would be sought to verify whether a suspect device had been used to download illegal material, and to take a copy for use in evidence.

    \item As most CSAM consists of streaming media originated in low-income poorly-governed countries~\autocite{Bursztein2019}, and as anti-terrorism agencies want to arrest people watching beheading videos, the Listening Post would need the ability to sample images from video streams and make them available as evidence, in order to convict the viewers of such content. 

    \item In conversations about client-side scanning with NGOs, the European Commission sought a mechanism to automatically screen content on all devices, not just devices under suspicion. NGOs responded that this appears to be in conflict with the European-law prohibition on warrantless mass surveillance.  

    \item Agencies in some countries could demand the ability to use the Listening Post to launch a privilege-escalation attack on a target's device so as to install a remote-access Trojan, on production of a warrant.\footnote{The UK Investigatory Powers Commission, for example, granted the National Crime Agency a `targeted equipment interference' warrant to empower them to install a remote access Trojan on all phones in the UK running the EncroChat app. The legality of this warrant was confirmed by the Court of Appeal.}
\end{enumerate}

The cumulative effect of these capabilities is to give the agencies even more powers than they have against server-based communications, such as Facebook Messenger. 

\subsection{Code Origin}
All scanning for suspect content, regardless of how it is done---hashes, perceptual hashes, or machine learning---requires access to frequently updated data. 
This may be a list of hash values or it may be a new set of parameters to a machine learning model. 
We will refer to such data, along with other parameters such as the server to which suspect content should be reported, as the signature data.

There are several jurisdictional problems associated with signatures. 
Each country may want to have its own, if only because each country may have its own criteria for targeting content.
This poses a difficult technical and jurisdictional problem: how should a client device obtain the proper signatures?
Conceptually, one can envision building in a master list of geographic areas and the proper URLs from which signatures are obtained, but political realities make that difficult, too.
Who, for example, supplies the signatures for Taiwan or the West Bank?
And who controls the master list?

Another vitally important question is who writes the code to do the client-side scanning. Might it be be a government agency, an app developer, or an operating system developer? All have their challenges.

It is unlikely that government agencies will supply code to be integrated into applications. 
It takes specialist skills to write code that runs robustly on the tens of thousands of machines that make up a communications service at a large modern service provider such as Google or Microsoft or Facebook.
Applications vary tremendously, differing in internal architecture, programming language, memory usage conventions, performance bottlenecks, and more. 
Even an engineer moving from one of these firms to another may take several months to become productive, and need their code checked by colleagues.
%(Performance is especially critical when dealing with streaming media.) 
For similar reasons, neither governments nor their defence contractors should expect to be able to write client-side scanning code for each individual application. 

The jurisdictional questions (see  \autoref{sec:jurisdiction}) make this even more difficult; dozens of governments would want their engineering teams to be building code into the servers and apps of the main service providers. 
Testing all this code properly would stretch the resources of even the largest service provider.
Even in major tech companies, effective engineering teams are small---in Bezos' words, small enough to be fed from two pizzas.
And would governments want rival governments to build code into services on which their citizens rely, or even to trust a defence contractor that worked for many other governments?

The trust issues would be even more severe if a listening post were inserted at the operating-system level. 
OS vendors would object very strongly to using government-provided code.
They would need to assure themselves that the installed code contained no other malicious functionality.
Experiments have shown that it is virtually impossible, even for experts, to detect this\footnote{Nicole Perlroth describes an exchange between James Gosler of Sandia National Labs and Robert Morris, then Chief Scientist of the NSA's National Computer Security Center. Morris was certain that the NSA could find any back doors in a code base of less than 10,000 lines---but his elite team could not find the traps that Gosler buried in a program of less than 3,000 lines. \parencite[Chapter 7]{Perlroth2020This-is-How-The}}.
Historically, OS vendors have objected very strongly even to being required to include government-mandated surveillance functionality, from Microsoft in the 1990s to Apple in 2016.

One possible outcome is that governments might make available a set of signatures for a pre-specified algorithm, defined at the level not of the operating system but of content filtering in the input and output of a communications app. 
This might evolve into an international standard, like the ETSI standards for wiretapping. Note that these standards are proven insecure~\autocite{athens-affair,Cross2010Exploiting-Lawf,rfc3924}.


There are several potential risks here. One is the nature and sensitivity of the signatures. 
As noted,  it is most likely that there will be many differing signatures as different jurisdictions apply different definitions of targeted content.
Many of them will be considered sensitive for various reasons.
If a file of perceptual hashes for a CSAM filtering app such as PhotoDNA came into the hands of adversaries, they could rapidly work out how to tweak images to evade it, or to cause innocuous images to report false positives, swamping the system. 
The same holds for machine-learning models; if they fall into the adversaries' hands, they are exposed to `white-box' attacks, which are generally more powerful than `black-box' attacks that merely probe a remote system and use its responses to evolve attacks.
Where governments pretend to be scanning for porn but are actually trying to censor pro-democracy activists, the compromise of a signature file containing lists of relevant keywords or other selectors will expose the ruler to personal embarrassment.

Yet while iPhones provide reasonable technical protection of one app against other apps on the same phone, and even against the phone's user, this is not the case with Android.
The majority of Android phones are not patched up-to-date because the OEMs generally do not ship patches for Android versions that are not currently on sale~\autocite{SEv3}.
If, therefore, client-side scanning tools are made available in Android versions of popular apps such as WhatsApp, it is not clear how any signatures therein can be protected from capable adversaries.

Although the proponents of client-side scanning talk mostly about illegal images, their documents have from day one assumed the scanning of text too, as was also the case with China's Green Dam. Text scanning creates a clear risk of the scanner being used not just to find illegal images but for censorship or to identify dissidents~\cite{EFF2020}.

\subsection{An increased attack surface}

Client-side scanning changes how attacks can happen. If, as proposed, the scanner must be installed on all devices policymakers must consider adversaries who might abuse the system for different objectives. This section gives a brief summary of potential adversaries, considering their access, motives, and capabilities.

We begin by delineating the deployment and operation flow of client-side scanning: 
%
\begin{enumerate}
    \item A reference client-side scanning implementation is developed, either publicly or released to select industry partners under NDA.
    \item Implementers translate the reference implementation to their own code base.
    \item Updates to the reference implementation are eventually incorporated into production code; this code is updated according to the normal update cycles---Windows Update, Apple's App Store, etc.
    \item The running code periodically updates its machine-learning model or perceptual-hash list, from the appropriate source.\footnote{Spam filters run by commercial email service providers are trained daily, but spam runs in the billions of messages per day.  These days spam is generated by a small number of large gangs who react to changes in filters daily. If producers of targeted content were to react to client-side scanning in the same way as spam producers, the scanners would need to be updated as frequently.}  

    \item When downloaded content is matched, the suspect content is uploaded for secondary screening by the service provider, followed by manual examination and, if need be, by a referral to the appropriate authorities. Again, this will vary by jurisdiction; in the US, suspected CSAM would be sent to NCMEC.
\end{enumerate}


Who supplies the CSS code matters as it constrains who can insert (hidden) functionality. While risks of misuse always exists, the attack surface can be reduced. For instance, if the code is written by a service provider, it becomes more difficult for a government agency to stealthily insert hidden functionality. In particular, the operational flow may set limits on what adversaries can and cannot do. Consider the following attack possibilities:
\begin{description}
\item[Remote code execution (RCE)]
RCE is improbable. 
As outlined above, platforms are unlikely to use government-supplied code directly, and for more reasons than security. 
%The risk from signature databases seems comparable to ordinary web browsing, unless the postulated scanning language is too powerful.
\item[Routine tracking] Ordinary device tracking is enhanced by the need for updates to ML models or hash lists.
However, given the scale of updates---there are literally billions of devices in the world, all of which would need regular updates---these updates would have to be done via the regular app update mechanism. As most modern devices are regularly polling for routine app updates, the incremental risk is low.\footnote{As most Android phones are out of support and do not get OS updates, any filters installed at the OS level could potentially be evaded by people buying insecure second-hand phones. But incentivising people to avoid patching is bad for a nation's security.}
\item[Targeted tracking] When a content scanner detects potentially suspicious content, that content is uploaded for screening at the service provider followed by possible manual inspection, along with enough information to identify and track the suspect device.
This is, of course, the entire goal of CSS, but it points to a crucial vulnerability if the signatures
are controlled by corrupt parties: CSS will identify people viewing innocent content that initially appears similar to targeted material.

There is another aspect to consider: what sorts of content can be scanned? %A CSS model or hash database designed to scan only images will be unable to scan text and hence unable to pick up words that some government considers improper. 
Currently the discussion is only about scanning images and videos; if CSS were to be extended to include text, that would create a major risk of censorship.

\item[Planted content] There will be critical risks from content tailored to trigger that signature.

\item[Filter configuration]
What ML model or perceptual-hash list should a device use? 
If an adversary has control---possibly legitimate---over a filter, they can insert whatever they wish. 
It is likely that each filter would point to the appropriate reporting station, such as a secondary screening server.
Thus one tactic for an attacker is to change which filter is loaded.
\end{description}

The question, then, is which adversaries can trigger which of these actions. 

\paragraph{A government.} Countries conduct surveillance on other countries and, in some cases, their domestic political rivals, whether at home or in exile. Reasons include espionage,  counter-terrorism, and political manipulation. 
Subverting a CSS process provides a new way to conduct these activities.

Governments will control the filters within their jurisdiction. Their simplest approach would be to control which filter is loaded by suspects. 
Alternatively, they could attempt to manipulate other countries' filters, whether via technical or political means.\footnote{As a technical example, for many years the US and German intelligence services covertly owned Crypto AG, a Swiss company that was the main provider of cryptographic equipment to non-aligned countries, thereby getting privileged access to traffic. As a political example, authoritarian rulers have often accused political rivals for terrorism and sought to put them on the Interpol red list.}

\paragraph{The system provider.} Both deliberate misuse and accidental leaking of data are commonplace, even from large and sophisticated tech companies. 
A compulsory surveillance mechanism could make this worse, because the increased complexity could increase the risk of security problems, while the necessity to support surveillance could shift incentives away from more secure mechanisms such as forward secrecy.

\paragraph{Rogue actors within trusted organizations.} Individuals within both law-enforcement organizations and tech companies have been known to subvert surveillance mechanisms, either for their own goals or as a result of coercion. 
Client-side content collection and filtering would provide a new attack surface which the organization might be both less able and less motivated to defend, because the attack would be conducted on citizens' phones rather than on a central organisational asset such as a messaging or filtering server.  

\paragraph{Organized-crime groups.} Although obviously a possible target of a surveillance mechanism, criminals including organized crime syndicates could also abuse it. If they can subvert it, they could use it to surveil other citizens or law-enforcement officers. If they can subvert the update mechanism, they could use it to install ransomware on hundreds of millions of consumer devices.

\paragraph{A family member, partner, or ex-partner.} Some of these parties control the devices of their targets; others merely control the infrastructure. 
They may frame someone by sending or receiving illegal material using their device and then denouncing them to the police. 
They may also take advantage of information leaked by the mechanism without necessarily being able to read all of it; for example, they might observe that a device was sending material to the cloud for secondary screening~\autocite{Levy2020Security--Threa}.

\bigskip

The benefits of mandating the installation of any surveillance mechanism on citizens' devices must be measured against the increased risk of compromise and use by an adversary, whether a foreign government or a criminal enterprise. 
Both actors might subvert employees of trusted organizations such as law enforcement and tech companies; they might also gain access by compromising these organizations' infrastructure, as seen in the Solar Winds case.\cite{}

%\emph{This is IMHO the largest and most serious risk.  Add some more examples of CCP or FSB surveillance of people in the US, Aus or Europe.  There are plenty, and I think the argument that we're making it easier is the strongest argument here.}

\subsection{Jurisdiction and Evidence}
\label{sec:jurisdiction}

The distributed nature of CSS will make issues of jurisdiction acute. 
Jurisdiction was an issue with key-escrow proposals in the 1990s, but did not become salient to U.S. policymakers while the main tech companies were American.  

A possible outcome would be that service providers have surveillance servers in multiple jurisdictions, and a means of deciding which server each app's LP must talk to. 
This will not be straightforward. First, users are mobile; millions of EU residents commute across borders. 
Second, states have different definitions of unlawful content.%\footnote{In 2000, the UK Regulation of Investigatory Powers Act required banks to provide keys or passwords in response to an order from a Chief Constable. Swiss law prohibited this. At least one US bank moved the administration of its European operation from London to Switzerland as a result.} 
Third, while some service providers collect enough data to have some idea where its users are, not all of them do.
Finally, people can use a VPN to appear to be in a different country.

Compare client-side collection with the case where a phone is seized from a suspect and examined following due process. 
Many countries also allow the mobile phones of travelers to be seized and examined at the border, even without due process. 
In such cases, standard forensic procedure is to image the device and analyze a copy. 
Investigators would not normally extract key material from its secure element or keystore, and would thus not be able to impersonate the suspect, which may be important from the viewpoint of evidence.

However, things are never simple with complex technology. 
A real problem is how to deal with cloud forensics, such the extraction by investigators' tools of a phone's Google master cookie, following which the tools download all the suspect's Gmail and Google Drive contents. 
The sort of concern that designers of a client-side collection system will have to foresee is this:  suppose an adversary offers the target a network connection that goes over a VPN to a different jurisdiction. 
For example, one country hacks a wifi point in a cafe frequented by people who work for a rival country's government. 
Unbeknown to them, they now appear to the service provider to fall under the attacking nation's rules, which can be crafted to their disadvantage.
The client-side scanner dutifully spots sensitive images and sends them off for `secondary screening' by a hostile intelligence service.

\subsection{The Scope of Control Mechanisms}

Client-side scanning is an overly broad technology for tackling the illegal-content problem. 
Governments have used control mechanisms to enforce a wide range of policies. 
Looking at several examples helps illuminate what kind of mechanisms are likely to be most effective.
\begin{enumerate}

\item With the prohibition on copying banknotes enforced by color copiers, scanners, and graphics-processing software, authorities found that they had to exempt open-source graphics software. If the banknote-detection software had been published, it would have become much easier to circumvent. Policymakers had to choose between an open-source exemption and a weakened mechanism; they chose the former.

\item Because of concerns that terrorists might use DNA synthesis technology to create bioweapons, some 80\% of synthesis machines screen for biohazards.  Active research is making this screening     technology both more ubiquitous and more privacy-preserving.\footnote{See \url{https://www.securedna.org/}.} 
Policymakers may decide that such screening is worth mandating, even if there is some leakage via open-source channels or serious contravention by rogue states.

\item The most pervasive control mechanism may be the global system of anti-money-laundering controls, which have proliferated since 9/11. Banks are reluctant participants, but spend a fortune on compliance because egregious violations can carry ten-figure fines. The AML regime is startlingly inefficient. It blocks less than 0.1\% of illegal money transfers, while compliance costs exceed blocked criminal funds a hundred times over (cite Pol).

\item Another widespread control mechanism is toxic content filtering. By this we mean not just explicitly illegal material such as phishing, sex abuse and beheading videos, but spam, hate speech, animal cruelty and much else. 
The larger social-media firms use machine-learning models, but abusers game the systems constantly, and there are many difficult edge cases. 
As a result, the models need to be retrained constantly and are backed up by tens of thousands of human moderators who adjudicate edge cases.
These controls impose costs of billions of dollars on businesses.
\end{enumerate}


Within more diverse and complex ecosystems, whether a specific type of abuse is removed efficiently depends on the context and the incentives. 
Service providers complain of the costs and complexity of moderation, but remove some kinds of toxic content where failure to do so would attract large fines. 

However, the effective control point often does not lie with the tech companies. 
The classic example here is sex-abuse material. 
The largest purveyor was the Canadian website Pornhub, which was brought to heel after a campaign by \textit{the New York Times} caused Visa and MasterCard to cut off its payment channel.

Any control system needs constant updates as authorities learn of new types of target material. 
Anyone---an individual, an agency, a government---with the power to update the client-side control system has a powerful form of  access. 
With update access to the phone platform, they could also potentially compromise all control technologies used by other agencies including those of other governments. 
Indeed, such access could be abused in a supply-chain attack to install ransomware at scale. 
Even if the agency had only read access to all data flowing through a platform, this could still be abused to capture second-factor authentication codes sent to a target's phone---and hence to compromise bank accounts. 
Making such a capability available to all the world's tens of thousands of police forces in some 200 countries would have unacceptable consequences for security.

Surveillance tools have often suffered from mission creep, starting with a very limited set of reasons in which they were to be used, and then having the reasons vastly increase. 
Again and again, access sought and justified by talking about terrorism ends up being used to investigate minor crimes as well.\footnote{One example is the number of serious crimes under which a wiretap order can be promulgated in the U.S. Under the original act in 1967, Omnibus Crime Control and Safe Streets Act, only twenty-five types of crimes constituted a serious crime for which a wiretap warrant could be obtained. As of this writing, the list is close to one hundred. Another is the UK Regulation of Investigatory Powers Act; sold to parliament in 2000 as a counter-terrorism tool, by 2006 there was a public row about whether its provisions could be used to investigate dog fouling.}

In some jurisdictions, such as the EU, the courts have ruled against bulk surveillance without warrant or suspicion; in others, such as Australia, they have not done so; in yet others (such as China) such surveillance is mandated. 
It is to be hoped that the EU is a sufficiently large market to prevent device vendors enabling surveillance by default; it is to be feared that China is a large enough market that surveillance may at least be installed. 
Policymakers who fear Chinese surveillance sufficiently to block Huawei from 5G networks should, if they were consistent, insist that bulk surveillance capabilities not be built into the devices on which we depend.  
After all, many, if not most of them, are made in China.

This clarifies the need for many of the Carnegie principles, providing a strong argument why technological infringements of rights must be limited and purpose-specific. 
The limitation can be functional (e.g., stop the copying of banknotes) or by target (e.g., requiring warrants to install malware on the phones of criminal suspects). 
Providing a mechanism that could be abused to install malware on everybody's phone is a bridge too far.

\subsection{Summing Up: Security and Complexity}

Cybersecurity is not becoming any easier.  
As systems become more complex, attackers find ways to exploit the complexity.\footnote{A recent example is the discovery that modern CPUs are vulnerable to attacks such as Spectre and Meltdown, which exploit the speculative execution used to optimize CPU performance.} 
We face alarming dependency on a growing number of major points of failure, including not just our two basic designs of CPUs and our handful of operating systems, but now also three large cloud-service providers and our Internet interconnection infrastructure. 
The SolarWinds attack showed that a single database performance- management tool could have exposed 18,000 organizations when it was compromised by the Russians. 

Creating another major point of failure by building a backdoor into iOS and Android (for example) would be a substantial addition to strategic vulnerabilities---especially as its exploitation would not be limited to U.S. agencies. 
Every other country could demand a key, as a condition of market access for the phones in question.
In 2010, India insisted that Blackberry have a messaging server in India for Indian users, so that their police and intelligence services could get access without going through Canada~\autocite{Blackberry2010}; and in 2021 it emerged that China had required Apple to move its Chinese iPhone users' data to three `iCloud' data centres operated in China by companies owned by the Chinese state~\autocite{Nicas2021}.

With these risks in mind, a workable policy is unlikely to be an off-the-peg technological `solution', but rather a process whereby controls are refined over time in the light of experience. 
Because insider threats are inevitable, a convincing answer will be needed in each case to the question of ``who will watch the watchmen.'' 
Continuous technical review and oversight must be part of any proposal.
Finally, security mechanisms must be both effective---i.e., not leak too much---and the least intrusive way of achieving the stated goals.  

\section{Core Security Principles}

Most modern control mechanisms have an information-processing component, with both the underlying technology and any security mechanisms based to some extent on software. 
We therefore need to consider core principles of information-security engineering.

\subsection{Managing Risk via Architecture}

While good engineering can reduce the risk of compromise, it cannot be eliminated entirely. 
People make mistakes, take shortcuts, or succumb to corruption; devices fail, are corrupted by malware, or have design flaws that emerge over time. 
Designers of secure systems therefore aim not just to prevent harms, but also to limit the scale and scope of those harms.
This is expressed via numerous security policies that have evolved in different sectors, and that have driven the security architectures on which these sectors rely. 
Two of the best known are those used in government and in banking.

\begin{itemize}
\item Multilevel security and compartmentalization are used by law enforcement and intelligence agencies, both to prevent surveillance product being taken out of the organization's systems, and to limit the number of officers with access to it.
\item Shared-control policies are used in financial services to ensure that transactions of consequence are authorized by more than one officer.
\end{itemize}

Both of these approaches have developed over many years and assume that the main threat comes from insiders. 
Both try to ensure that the disloyalty or incompetence of one officer, or some small group of officers, will not have catastrophic consequences. 

Good design requires clarity about both the control objectives and the failure modes; these in turn depend on a clear understanding of the threats, and the consequences of failure.

% Another problem with mandatory use of ML is the possible introduction of inappropriate biases.  While ML filters are relatively easy to build, we lack a good understanding of the detailed criteria a filter may use.  For instance, filters that have been used to evaluate the creditworthiness of loan applicants or help judges decide prison sentences have been found to include racial biases. (Cite Bryson et al.)

% This lack of understanding of an ML filter's criteria also creates a lack of accountability.  Filters can be overly broad; they may also unfairly target particular individuals (whether by accident or design) without any clear evidence that this has been done. It is not clear how ML filtering can be built to respect the specificity and limitation principles described above.

% (Something here on scale? Spam filter experience; and how do you deal with 28bn WhatsApp messages a day? Anything above one in a million false positives and you'll be working hard...)

% Finally, control of the filters establishes control of the information spigot. While filters could be tuned to trap only narrowly-targeted materials on a small set of devices, there is nothing to stop them from being used as a tool for mass surveillance once they are deployed at scale.  And the lack of transparency of the filters themselves makes it extremely difficult with current tools to engineer systems that will give assurance to the public, to lawmakers, and to courts of the breadth, the scope, the specificity and the fairness of this surveillance.

%\subsection{Enforcing Policy Through Technical Means}


There are three primary classes of actors: technology providers, governments and users.
%\begin{itemize}
%\item \textit{Technology Providers}, including cloud platforms such as Amazon's AWS, Microsoft Azure, and Google Cloud; mobile-device platforms such as Android and iOS; online services such as Facebook and Gmail; and apps for encrypted end-to-end communications such as WhatsApp and Signal.
%\item \textit{Users} who may be empowered or exploited by such technology; 
%\item \textit{Government and standards organizations} who regulate technology to meet policy objectives; and
%\item \textit{Adversaries} who seek to subvert these technologies for their own purposes.
%\end{itemize}
%Users are generally motivated by personal needs, providers by their business objectives, and government by a desire to promote the public good: in theory, regulation tries to preserve technology's benefits while limiting the damage. 
All three may act in adversarial ways, both individually and in collusion. 
Providers may capture government regulators; governments may pressure providers; providers may exploit users; users may commit crimes; and governments may seek tyrannical power over users. 
Any of the parties may be corrupted, and technology may be used for good or for evil. 
Both providers and governments have internal controls to minimize the risks of abuse by powerful insiders, whether these are adversarial individuals or devices that have been taken over by external adversaries. 
However, as the risk is never zero, we need to consider carefully how to limit the damage that can be done by an insider, whether in a government agency or a firm.

\subsection{Effective, Limited, and Purpose-Specific Controls}

Some pervasive controls can be limited to specific purposes, and also made more effective, by implementing them in specialized equipment or apps. 
In the examples we mentioned above, software may be either distributed in devices (e.g., banknote copy prevention, drones, contact-tracing apps) or run on central services (e.g., curfew tags). 
Purpose-specific design also limits the possible damage if the mechanism or its operators are compromised.

%Controls that cannot be located in a specific device, and are instead deployed as software on people's phones, should be in a specific app rather than in the platform. Otherwise, the risk that the entire device can be compromised is simply too high. 


%Many control mechanisms existed before software, and some can be implemented using paper if need be\footnote{For example, while you needed a permit on your phone to go food shopping in Athens during the COVID lockdown, in Paris a declaration on paper sufficed.}. However the great majority are nowadays implemented substantially in software. 

%Control mechanisms may prevent certain actions completely (geofencing, speed limiters, toxic content dissemination), warn the user or others (contact-tracing apps, drone radio beacons), alert authority of a targeted action (curfew tags, AML suspicious activity reports), or create a log so that a targeted action can be investigated after the fact (tachographs). 
%While the role sought by government is mostly to observe and, in a minority of cases, to block targeted actions, it does not usually seek to alter or initiate actions\footnote{While there has been some action against violent online political extremism of the Islamist variety, there has been little against the right-wing variety, with the notable exception of Amazon's termination of service to Parler. Where violent online political extremism is promoted in a jurisdiction by allies of its government, social-media firms rarely prioritise its removal.}.

However, where controls with less clearly circumscribed aims are embedded in multiple places in a variety of services, they tend to be less effective---an illustrative example here being measures taken against money laundering. 
The world's payment systems are very complex, and `money laundering' covers a multitude of sins---from petty tax evasion by the self-employed, to extracting the proceeds of cybercrime using cryptocurrency, through major securities fraud, and the theft of national wealth by corrupt ruling elites, to the evasion of international sanctions.
Broad surveillance powers over payment systems can help target high-profile individuals of interest to governments, but do not generally lead to effective enforcement against the millions of minor offenders. 
The money-laundering reporting requirements generate such a firehose of `suspicious activity reports' that they cannot be used to drive enforcement, but merely as a reference after the fact when some individual or firm is suspected on other grounds.
The effect of the controls more generally is that innocent citizens can find their bank accounts blocked when they try to do large transactions such as cashing in a pension or buying a house, or even for no reason at all.
So a deep question is whether a control measure is intended to target some specific behavior, or to target specific individuals.

\subsection{Can Client-Side Scanning be Purpose-Limited?}

The UK's draft Online Safety Bill would grant the regulator the power to compel the provider of any new technology that enables people to communicate with each other to install an `accredited' surveillance or censorship technology. 
If it refuses, the regulator may penalize its infrastructure providers, and even require ISPs to block its service.
This direction of travel creates a risk that toxic content management will over time develop into a transnational bureaucracy, just like the anti-money-laundering ecosystem.
If that pattern is followed, it will be mostly ineffective, widely resented, and extremely expensive.

Although child protection and terrorism will be the justification, regimes will use these systems to control political discourse, stigmatise their rivals, and defeat their enemies. This leads us to the policy issues.

\section{Core Policy Principles}

%((This section needs to actually discuss the adherence of client-side scanning to core principles. Right now it is a simple recitation of those core principles. --Bruce))

Making judicious and responsible choices about surveillance technologies is done best by beginning with the principles that organize a society's choices.
Those countries that enjoy democracy and the rule of law have long restricted the surveillance powers of law enforcement and intelligence agencies, by prohibiting some kinds of surveillance and by restricting others using warrant mechanisms.
%How should these develop in the context of access to the growing diversity of communications available through mobile phones and other devices?
%The situation we face today, with increasingly serious threats to digital assets by governmental and non-governmental actors, and growing public use of a diverse set of apps that protect user privacy using cryptographic technologies---have both similarities and differences with the challenges cryptography has posed in the past.  

In considering how to guide policy to prevent the distribution of targeted content, we turn the 2019 Carnegie study, whose participants included former senior members of the U.S. government and experts from industry, academia, and civil-society organizations~\autocite{CEIP2019}.  
U.S. law enforcement had recently lobbied about the problems posed by investigations into locked mobile phones, the Carnegie study focused on that aspect of encryption. 
One of its key findings was a set of core principles to guide technical proposals for law-enforcement access to encrypted mobile phones. 
These principles are also applicable to client-side scanning as they provide authoritative guidance for surveillance mechanisms for communication devices~\autocite{CEIP2019}.\footnote{We are discussing the Carnegie principles in the order most suited to the client-side scanning issue; the principles were in no particular order in the original report\autocite[p. 20]{CEIP2019}.} 

Earlier we noted the serious security problems raised by client-side scanning. 
Because client-side scanning is intended to be used on all devices, it would violate the:

\begin{description}

\item{\bf Focus Principle:} The capability is designed in a way that it does not appreciably decrease cybersecurity for the public at large, only for users subject to legitimate law-enforcement access.
\end{description}


The combination of broad use of client-side scanning with the ability to change the particulars of what constitutes `targeted collection' means that client-side scanning also violates the:

\begin{description}
\item{\bf Specificity Principle:}
The capability to access a given phone is useful for accessing only that phone (e.g., there is no master secret key to use), and that there is no practical way to repurpose the capability for mass surveillance, even if some aspects of it are compromised.

\end{description}


As noted earlier, it is likely that various types of attack against client-side scanning would enable criminals to learn enough about the models or perceptual hashes to defeat them, thus becoming able to disseminate CSAM or falsely stigmatize others for its possession. 
Meanwhile the client-side scanning would continue to work against all other users, raising significant privacy and security risks. 
We argue that current forms of the technology violate the: 
 
\begin{description}

\item{\bf Utility Principle:}
The proposal can meaningfully and predictably address a legitimate and demonstrated law-enforcement problem.
\end{description}

There is no reason to believe---and many reasons to doubt---that advances in client-side scanning will improve the situation.

Because client-side scanning operates on {\it all} phones, particularity of searches is absent. Use of the technology violates: 

\begin{description}


\item{\bf Authorization Principle:} The use of this capability on a phone is made available only subject to duly authorized legal processes (for example, obtaining a warrant).

\item{\bf Limitation Principle:} The legal standards that law enforcement must satisfy to obtain authorization to use this capability must appropriately limit its scope---e.g., with respect to the severity of the crime and the particularity of the search.

\end{description}

One of the fundamental principles in U.S. surveillance law is oversight, as well the ability of the accused to see the data the government has against them; this can be found in the {\it Wiretap Act}\footnote{the U.S. government publishes an annual report listing all criminal wire taps conducted each year including such information such as how long the wiretap existed, how many incriminating conversations were collected how many non-incriminating, what the most serious crime being investigated was, etc.} and in the {\it Foreign Intelligence Surveillance Act.} 
Thus, the Carnegie report also includes: 

\begin{description}

\item{\bf Auditability Principle:} When a phone is accessed, the action is auditable to enable proper oversight, which is eventually made transparent to the user (even if in a delayed fashion, due to the need for law-enforcement secrecy).

\item{\bf Transparency, Evaluation, and Oversight Principle:} The use of the capability will be documented and publicly reported with sufficient rigor to facilitate accountability through ongoing evaluation and oversight by policymakers and the public. 
\end{description}

We note that these principles have broader applicability than for just the United States. 
In the European Union, for example, rights such as privacy are entrenched in the Charter of Fundamental Rights, and can be overridden only by law and in ways that are both necessary and proportionate. 
Thus, for example, the lawmakers cannot simply say, ``Because of  terrorism, the police may disregard right X in manner Y.'' 
It must be established that Y is proportionate and necessary in the fight against terrorism, otherwise the European courts may strike down the law. 
Infringements of rights must be limited and purpose-specific, which aligns extremely well with the Carnegie principles.

The Carnegie report examined the issue of developing technology to obtain content from devices. 
Employing client-side scanning technologies essentially sets up a user's phone as a surveillance device, raising additional surveillance concerns. 
Thus we recommend augmenting the Carnegie report recommendations with: 
\begin{description}
\item{\bf No Bulk Surveillance Principle:}
Communications devices and computers should not be designed to function as surveillance devices.
\end{description}

Some of this point is inherent in the specificity and focus principles, but given recent proposals for client-side scanning, we believe this principle needs to be called out explicitly. 
In particular, governments should not require that surveillance monitors be built in to our phones and computers to detect if or when we do something `wrong'. 
Nor should industry build systems that do so. 
Law-enforcement surveillance should continue to be targeted for a specific purpose, as in the past.

However, existing and proposed laws in several countries allow governments to make secret orders, instructing communications service providers to install locally accredited technologies for censorship, surveillance, or both. 
For users to understand what is and is not technologically possible, detailed descriptions of device communications protocols should be available for public scrutiny. 
Without this, users will be even more fearful that surveillance systems have been installed secretly on the devices on which they rely to live their lives.

\begin{description}
\item{\bf Full Transparency Principle}
For full transparency, detailed descriptions of the design and implementation of content scanning mechanisms should be available for public scrutiny.
\end{description}

Without the ability to examine the code, there is no way to know if there is nefarious code in the scanner. However, mere access to the code is not enough. Good security engineering starts from a realistic threat model, and proceeds via a security policy that states the high-level protection goals, to a protection profile that sets out how these goals are met in a specific system. To command any confidence, an open design is essential, and this means openness about the whole engineering project, from threat model through security policy to protection profile and assurance requirements.

We therefore recommended that anyone proposing regulations for client-side filters or other exceptional access should present concrete technical requirements---which industry, academics, and the public could analyze for technical weaknesses and hidden costs.
Where such filters or other exceptional-access mechanisms are to be installed by default on consumer devices, rather than on targeted suspects following a warrant, should also explain how the following issues will be dealt with:

\begin{itemize}
    \item the specific purpose of the exceptional access and how the mechanism will be limited to this;
    \item the false-positive and false-negative error rates, the costs of such errors, and how they will be dealt with;
    \item interaction with chat messages that have existing legal status from personal health information (HIPAA/GDPR) to diplomacy;
    \item interaction with jurisdiction;
    \item whether the technical design supports or undermines the governance and accountability mechanisms;
    \item who will update the filters, and how often;
    \item how their operation will be monitored for legitimate purposes, respect for other legitimate interests, fairness, and effectiveness; and finally
    \item who will bear the costs, and how their incentives will be aligned.
    %\item what else?
\end{itemize}

While specific signature data such as keyword lists, perceptual hashes and ML models may need to be kept from adversaries, even they must be auditable, and not just by the big audit firms; they must be available for academics who sign NDAs to study. 
As for the scanning mechanisms themselves, their design and implementation must be open to all.
Only with such information can citizens assess whether such a technical proposal is politically acceptable, and indeed consistent with fundamental rights such as the U.S. Constitution, the EU Charter of Fundamental Rights, and the European Convention on Human Rights.

\section{Conclusion}

We have taken a careful look at various means by which law-enforcement agencies can monitor and regulate actions on user devices.  
Prior efforts over past decades have focused upon providing law enforcement direct access to user keys or data, and these approaches have failed for reasons detailed in past reports\autocite{1997Report,KUD}.  
A more nuanced approach has arisen in recent years, wherein user devices effectively monitor themselves and report and/or block only targeted materials.

While this self-monitoring approach may seem appealing, technologies to implement self-monitoring introduce substantial technical problems both in their effectiveness and in the risks they pose to users' security and privacy.  
Client-side scanning for targeted materials inherently weakens the privacy guarantees of existing systems by breaking the assumptions that underlie the cryptographic models in common use.  
It can also threaten the security of user devices, by violating the basic access mechanisms used to protect these devices.

Narrowly targeted surveillance mechanisms such as `lawful hacking' are in regular use today.
In these cases, our societies generally accept that the targeted suspect will have their security weakened, and will in consequence be more vulnerable to third-party attacks. 
However, attempts to scale these methods to the broader population threaten not just the integrity of a few devices, but all our devices---and the important services they give us---in the absence of any probable cause for interference having been determined by a court. 

In the 1970s, in response to decades of NSA, FBI, CIA, and Army excesses of surveillance of Americans exercising their constitutionally protected rights, a U.S. Senate Special Committee observed the grave danger to the state of such scrutiny: 
\begin{quote}
  Persons most intimidated may well not be those at the extremes of the political spectrum, but rather those nearer the middle. Yet voices of moderation are vital to balance public debate and avoid polarization of our society.\autocite[p. 307]{United-States-Senate1976Intelligence-Ac}
  \end{quote}
Client-side scanning will ensure neither society's security nor liberty, but instead may seriously endanger both.

%In short, the current proposals are infeasible, create serious insecurities in core communication devices, empower current major stakeholders and discourage competition, ...

%``A huge insecurity that affects the whole of society.''

%- Link with the theme that this is just one more instance of the general pattern sketched out in Sec 2 - i.e. of introducing surveillance mechanisms only to discover they can be abused for a purpose not matching the intended one.


\section*{Appendix: A History of the Crypto Wars}

The spectacular success of the UK and the USA in reading encrypted German and Japanese traffic during World War II led the USA and its allies to try to retain access to the world's military, diplomatic, and intelligence traffic in various ways.
These included both overt strategies, such as cryptographic export controls; and covert strategies, such as the secret ownership by U.S. and West German intelligence agencies of the cryptographic-equipment firm Crypto AG in Switzerland.

\subsection*{Early Years}

These strategies gave the allies exceptional access to the communications of many other governments, but came under stress in the 1970s for two reasons. 
First, the invention and proliferation of automatic teller machines (ATMs) created a need for private-sector encryption, and IBM developed the Lucifer algorithm for Lloyds of London in 1971. 
As a result of the 1974 Privacy Act and increasing storage of personal information of Americans in government databases, the U.S. government came to accept that there was a need for approved cryptography outside of national security; this included unclassified use in government. 

The National Institute of Standards and Technology (NIST)\footnote{At the time, this organization was called the National Bureau of Standards, but for simplicity we will refer to it as NIST throughout.} put out a call for a Data Encryption Standard (DES), and IBM responded with a block cipher algorithm based on its ATM work. 
The IBM algorithm had a 128-bit key; the National Security Agency (NSA) demanded that it be shortened to 48 bits; the eventual compromise was 56 bits\autocite[p.232]{nsa-history}. 
This was long enough to protect the PIN of a bank card issued in 1980 with a lifetime of two years, but too short for a government secret with a lifetime of twenty years or more. Entirely predictably, by the late 1990s Moore's law made it possible for private parties to break DES keys by brute force\autocite{descrack}. 
In this way, the U.S. government made available an algorithm that was strong enough for short-term commercial use, while deterring foreign governments from using it instead of Crypto AG's apparently more secure offerings.

The development of DES helped bring cryptography to the attention of academic researchers, leading to the development of public-key encryption, which had been previously discovered by GCHQ, and digital signatures, which had not. 
Despite the signals intelligence community's massive head start, academic researchers had now pulled ahead in some respects, a fact that alarmed the NSA. 
Its officials tried to get a right to prior review of cryptographic research being funded by the National Science Foundation (NSF), and wrote to the IEEE warning them that publishing cryptologic research might contravene the International Trafficking in Arms Regulations. 
This led to a public confrontation at the 1977 International Symposium on Information Theory, and disagreement between government departments. 
Eventually the NSA Director Admiral Bobby Ray Inman backed down, but the agency still seeks to influence the direction of academic research via government funding mechanisms.

The agency also continued to use export controls to limit the spread of cryptographic technology, as it was largely implemented in hardware devices in the 1980s. 
These controls allowed banks to buy cryptography to manage ATM PINs and keys, but let officials negotiate its use in other applications case-by-case. 
But control was undermined by the growing availability of software encryption on personal computers, and the growth of proprietary email and messaging systems. 
National-security officials foresaw that once these systems joined up via the Internet, the presence or absence of encryption would make a real difference to signals intelligence capabilities. 

In 1993, the NSA therefore persuaded the incoming Clinton administration to try to bring cryptography more firmly under government control, sparking the first ``Crypto War.''

\subsection*{Access to Keys: Crypto War I}

The U.S. government and some of its allies now started pushing systems that contained acknowledged backdoors. 
The opening shot was the Escrowed Encryption Standard and ``Clipper Chip.'' 
These were NSA proposals whereby encrypted traffic would be accompanied by a ``Law enforcement access field'' that allowed the authorities to decrypt the messages. 
One of us (MAB) showed how to defeat this mechanism by a trivial change to that field~\autocite{Blaze1994}. 

Governments' attempts to control cryptography came into conflict rapidly with big business, as the Internet was opened up to the public and companies rushed to establish e-commerce. 
Companies adopted SSL encryption for their websites, and private firms set up in business as certification authorities (CAs) to certify other firms' public keys, so that people could have some idea whose website they were dealing with. 
Governments reacted with a proposal to regulate CAs, insisting that every CA have a copy of each user's private key before certifying their public key. 
This way, law enforcement and intelligence agencies could trust the CA to hand over any key in response to a warrant. 
Such CAs were called ``trusted third parties,'' in the sense that they were trusted by the government to break trust with their customers. 
Governments also used export-control rules to limit the key lengths in the cipher suites that could be shipped with software for use overseas. 
Given the nature of the computer industry, such limits had pervasive domestic effects as well.

This struggle to control cryptography involved tussles in multiple private-sector systems. 
In some, governments used their regulatory power; GSM, for example, was fielded with a choice of weak encryption for trusted countries (A5/1, with an effective keylength of 43 bits) and even weaker encryption elsewhere. 
In others, export controls steered vendors to weak mechanisms: the Mifare contactless smartcard, used widely for public transit payments and in building entry control, had 48 bits, and many remote key entry (RKE) systems for vehicles were no better. 
Many networked systems simply sent traffic in the clear; some still do. 
Requirements in the 1990s that weakened cryptographic systems had impacts decades after the restrictions were lifted because of the need for backward compatibility in communications systems; thus browsers in the mid 2010s were subject to an attack that rolled encryption security back to 40-bit key lengths\autocite{Beurdouche}.

Two influential reports in the late 1990s helped steer the debate. 
In 1996, the National Academies of Science, Engineering, and Medicine published a consensus report, Cryptography's Role in Securing the Information Society, which observed, ``on balance, the advantages of more widespread use of cryptography outweigh the disadvantages.''\autocite[ p.7]{NRC96} 
In 1997 many of us wrote ``The Risks of Key Recovery, Key Escrow, and Trusted Third-Party Encryption,'' which analyzed the tensions between the demand by law-enforcement and intelligence agencies for universal, covert and immediate access to plaintext, and the societal need to protect the emerging digital infrastructures using cryptography. 
We explained that while it was often possible to design systems so that the owner could recover from the loss of a cryptographic key (as when banks keep backups of their cryptographic keys locked in their vaults), it did not appear to be possible to design systems that would allow the agencies universal exceptional access without unacceptable costs and risks. 
Some examples of the risks associated to enabling exceptional access are those arising from insiders in the following contexts: 
\begin{itemize}
    \item The relationship between confidentiality and integrity (whether officials with covert access to transactions could alter them);
    \item Authenticity (whether any official gets to impersonate anyone else);
    \item Accountability (who is able to audit who did what when);
    \item Jurisdiction (which of the countries involved in a transaction gets access to what); and
    \item Metadata (who can see who called whom when and where). 
\end{itemize} 

We are still paying the costs of the weak cryptography imposed in the 1990s. 
Countless thousands of buildings still have Mifare door keys that are easy to copy; car thefts are enabled by weak remote key-entry systems; and foreign adversaries can tap our mobile phone networks using the vulnerabilities we created in order to monitor theirs.

The Crypto War I battle ebbed when, in 1999 and 2000, the E.U and U.S. changed export-control regulations to permit stronger forms of encryption in products and services (though many democracies still have some restrictions in place and some, including Australia, still enforce them). 
In fact, the war never really ended; it only changed its form. 

\subsection*{Access to Servers: Crypto Wars II---The Snowden Revelations}

In 2013, Edward Snowden revealed that the NSA was getting much, if not most, of its intelligence product from PRISM, a system that extracted information from services such as Gmail, Hotmail, and Facebook. 
As network effects centralised information flows in a handful of large firms, their servers became the agencies' natural access points. 
The agencies therefore used FISA and other legal mechanisms to obtain access, a process which they automated; PRISM was the result. Snowden also revealed that the NSA had spent \$100m per year to weaken commercial cryptography by interfering at multiple points in the supply chain: with research, with standards, with protocols, and with products.\footnote{The codename for this was Operation Bullrun. GCHQ had run a similar program, also named after a Civil War battle: Edgehill.}

The tech industry was also stung by the revelation that as well as getting customer data through the front door by means of warrants, the NSA was also getting it through the back door by wiretapping communications between company data centers. 
This prompted the industry to turn on encryption everywhere. 
Entrepreneurs and open source developers offered numerous end-to-end encrypted messaging apps. 
Millions of people started to use cryptography in everyday communications, because chat apps unlike SMS messages were free. The government response included claims of investigations ``going dark,'' which had also been made in the 1990s. 
This time, governments started with narratives about terrorism and money laundering, and then switched to talking about CSAM. 

In reply, an expanded group of us published ``Keys under Doormats'' \autocite{KUD}, in which we showed how law-enforcement scaremongering in the 1990s had been misplaced. 
The world did not go dark for investigators, who instead got access to a cornucopia of new intelligence sources and methods. 
We found that, because of the growing economic and social cost of the insecurity of the modern Internet environment, the damage that could be caused by exceptional-access requirements would be even greater than twenty years before. 
The complexity of an environment with millions of apps and globally connected services means that new law enforcement requirements would be likely to introduce unanticipated, hard-to-detect security flaws. 
And implementing exceptional access would have immediate negative security consequences by forcing developers to abandon modern ``forward secrecy'' design practices that seek to minimize the impact when systems are breached. 
We recommended that anyone proposing regulations for exceptional access should first present concrete technical requirements, which industry, academics, and the public could analyze for technical weaknesses and for hidden costs.

\section*{Appendix II---Other Control Mechanisms}

Here are some more examples of pervasive control mechanisms.

\begin{itemize}
\item One of the oldest pervasive control regimes is for commercial vehicles. 
Buses and heavy trucks in Europe are required to have a \textit{speed limiter} restricting them to 100kph (62mph) plus a \textit{tachograph} to enforce legislation on drivers' working hours (eight hours a day with one hour of rest, with nine hours permitted one day per week). 
The speed limiter is a hard control whose circumvention is an obvious crime, while the tachograph logs generate evidence that can be demanded by a traffic officer. 
In addition to this distributed logging, there may be central surveillance in the form of trucking firms' fleet management systems. However both firms and drivers are incentivized to cheat.

\item A road toll or urban congestion-charging scheme is typically implemented using \emph{automatic number-plate recognition} (ANPR) cameras that link to a vehicle-registration system rather than by installing surveillance software on people's mobile phones or by doing cellsite location analysis. 
ANPR is a more effective and limited technology. 
In terms of effectiveness, if phone monitoring were used instead, there would be an incentive for people to switch off their phones, leave them at home, or even use burner phones instead (potentially harming other law-enforcement objectives). 
In terms of limitations, the potential uses of plate numbers is much smaller than that of GPS or other localization schemes on which app-based tolling and congestion-charging could be built.
    
\item \textit{Curfew} and \textit{quarantine} mechanisms have been implemented as tags people wear, or as apps on their phones. 
They have been used for over a decade to monitor suspects on bail, and prisoners released on parole; during the pandemic they have been adopted in many countries to track people who may have been exposed to coronavirus infection, and to monitor self-isolation by people who may have been exposed or who have recently arrived in a jurisdiction. 
In the criminal-justice applications, apps or tags report to a central monitoring service, with violators of bail or parole conditions facing arrest. 
In the public-health applications, many countries used apps for coronavirus contact tracing with privacy mechanisms implemented by Google and Apple that limit the app to advising the user, rather than advising the public health authorities. 
Various countries also built centralised systems for enforcing lockdown and quarantine; during lockdown in Greece in spring 2020, people had to apply online for a permit to leave home so they could show it on their phone to the police.

\item \textit{Drones} are now cheap and are widely used in aerial photography, but are prevented from entering prohibited airspace, such as near airports. In consumer drones this is done using \textit{geofencing}: the drone uses GPS to know where it is. The USA and the EU have separate legislative programs to force drones to have radio beacons, so that operators who cause trouble can be identified. 
Professional operators are licensed. Abuse by capable opponents remains possible as the control mechanisms can be defeated by knowledgeable people. 
But they make abuse rarer; and by preventing hobbyists from buzzing an airfield by accident, they ensure that such abuse is an obviously criminal act. 
\end{itemize}

\printbibliography

\end{document}
\section{Omitted Text}

\section*{Abstract}
Public access to strong cryptography has been contentious since the mid-1970s. append
National security first tried to limit its use, then proposed key escrow. 
Later, law enforcement agencies pressed for ``exceptional access'' mechanisms to get plaintext by other means. 
None of these propositions found wide acceptance. 
Meanwhile cybersecurity risks have increased. 
Building on the success of machine learning in a variety of venues, some in industry and 
in government have recommended ``client-side scanning'' as the silver-bullet solution. 
We show here that this proposal is basically a variant of exceptional access. 
Even worse, it creates even greater security risks than previous proposals.

(Notes from early meetings)

\subsection{Policy and Technology Environment:}
(this includes feasibility of technologies and economic and competitive factors)[Note that this is a suggested condensation of deleted sections 3 \& 4 below.]

What are LE and intelligence agencies asking for?

What about the priorities and responsibilities of other agencies in government, from financial regulators to safety regulators? Relate the EU experience of the Cybersecurity Act, and the need for cybersecurity expertise in multiple other regulatory agencies. Who will do that? Note the GCHQ director's line that cybersecurity requires a `whole of government response'.

Not just prohibited content but prohibited transactions... Do we frame illegal vs targeted (e.g. `must be reported'), and content vs transactions? Need to explain that targeting can come from multiple government and private actors; this complexity cannot be ignored. It's not just wiretapping but anti-money-laundering and much else. Do we call these `control mechanisms' or maybe `pervasive control mechanisms'?

Technical feasibility and effectiveness of possible options

Ross on infrastructure

Can the access be limited to devices in LE custody?

Is this feasible?

What are the implications”

Economic and competitive impacts of providing/mandating these technologies

Can major actors continue to operate?

Experiences in Australia and U.K.

\subsection{Technical proposals since 2015}

{\bf Josh to put some stuff here on ML scanning; Ross and Carmela to review.}

Client-side scanning: to prevent uploading and downloading of prohibited media.

Describe technical requirements, then discuss security risks, many of which are the same as with key escrow. Limit to capability of client-side scanning. What are the new security risks? 

Weaknesses of federated learning. 

Who has access to client-side scanning, both in terms of what terms are entered into the scanner and who receives output from it?  How well locked down is this access? 

To what extent are the specificity and focus principles violated by enabling device-side scanning? 

Can the capability be expanded outside a jurisdiction (loss of specificity)?

How can device-side scanning be repurposed from one set of content (e.g., CSAM), so that it acts as a surveillance tool on the device? 

What's the role of the many side channels that exist in mobile phones? What about other devices such as smart speakers and cars? Which other technologies do we want to look at? 

Josh and Mike's list below is extensive, but we need to be mindful of Ron's point of not being outdated ten minutes after we publish. We should not discuss each of them.


\subsection{This part has been cut from the introduction.}
The purpose of this document is three-fold:

\begin{itemize}
\item
Address filtering proposal.
  issues in the debate that have surfaced since 2015.

\item
We expand upon the frameworks from the 2018 National Academies cryptography report and principles from the 2019 Carnegie report, extending them to include protection against surveillance:
We should not allow government to install surveillance monitors in our phones and computers to detect if/when we do something "wrong".

Do we want to add: For full transparency, In addition, for full transparency, detailed descriptions of device communications protocols should be available for public scrutiny. Examine new technical proposals, including client-side scanning, --- and analyze for security and efficacy.

\end{itemize}

\subsection{Pervasive Policy Enforcement Mechanisms}


\subsection{Removed as Not Relevant}
In addition to these complexities, it is to be expected that law-enforcement and intelligence agencies will also make some or more of the following further demands.

\begin{enumerate}
    \item We expect that the agencies in many countries will demand access to live message traffic, so they can handle not only crimes already committed but also live cases involving immediate threats to life\footnote{In 2020, French and Dutch police installed malware in 20,000 phones running the EncroChat app, which was widely used by drug dealers, and this led to hundreds of arrests. The UK Court of Appeal ruled in the test case that a warrant under the Investigatory Powers Act for `equipment interference' enabled the police to collect both stored data, and data intercepted from the device on the fly.}.
    \item The agencies in many countries will demand access to the cryptographic keys used to secure VOIP and video calls so they can implement wiretap warrants.
    \item We expect that the agencies in some countries will demand an LP in the device platform as well, in order to collect device unlock passwords for later forensic use\footnote{This demand was already made by the FBI in respect of the San Bernardino attacks.}, and location data such as cellsite IDs and GPS coordinates so that suspect devices can be traced to individuals\footnote{Comparing devices' cellsite location history is how one finds burner phones, by associating them with identifiable devices carried by the same suspect. This technique was disclosed by Snowden and is now a standard operating procedure of police forces worldwide.}.
\end{enumerate}

Moved from the "Adversaries" section:

Yet some within the intelligence community are pushing for pervasive on-device surveillance. GCHQ's pitch document `AI for national security: online safety' sets a goal of:

\begin{quotation}``Providing tools and techniques to identify potential grooming behaviour within the text of messages and in chat rooms; highlighting the exchange of illegal images and tracking the disguised identities of offenders across multiple accounts; searching out and discovering hidden people and illegal services on the dark web. AI could also enable us to help law enforcement infiltrate rings of offenders and bring them to justice.''
\end{quotation}

So the filter code in your phone won't just be looking for illegal pictures. GCHQ goes on:

\begin{quotation}``AI tools can also be trained to analyse seized and intercepted imagery, messages, other forms of internet content, and chains of contact, to support investigators in the identification of victims and discovery of accomplice offenders. AI running across both content and metadata could also protect our analysts from unnecessary exposure to traumatically disturbing material.''
\end{quotation}

We do not pretend to have easy solutions to complex problems; we simply ask the reader to be sceptical when such claims from the intelligence community's leaders and lobbyists.

\section{Deprecated Executive Summary written by Carmela and Susan}

Public access to strong cryptography has been contentious since the mid-1970s. National-security forces tried to limit its use, then later law enforcement agencies pressed to do so. Many proposals have been suggested: key escrow and ``exceptional access'' mechanisms; none have found wide acceptance. Now some in industry and in government are advocating ``client-side scanning'' as a silver-bullet solution to the encryption quandary. 

Client-side scanning is hailed as a perfect solution that enables monitoring while leaving security and privacy intact. Instead of weakening encryption, or providing law enforcement with back doors, client-side scanning enables on-device analysis of data \emph{in the clear}. If targeted information is detected, it is revealed to the enforcement bodies. Otherwise, the use of client-side scanning neither weakens nor prevents the use of end-to-end encrypted communications, guaranteeing that non-criminals’ messages remain confidential.

We show here that, contrary to the promise of an acceptable security trade-off, client-side scanning introduces serious risks to the security of ordinary  users and to the information infrastructure as as a whole. This stems from the fact that in order to accommodate changing law-enforcement requirements, the content-identification needs can be arbitrarily complex, may change over time, and effective enforcement may often require them to be private. The main advantage of client-side scanning---the fact that it can be done privately, on the client device---is thus a direct cause of its main weaknesses. Due to the insecurity of user devices, the surveillance and control capabilities provided by client-side scanning cannot be owned by those deploying it, but are potentially available to any adversary, e.g., criminals or enemy nations, that can compromise the device or any entity in the chain that sets or updates the scanning policy. Resisting attempts to spy and influence non-criminal citizens is possibly the highest priority of our national security: client-side scanning does exactly the opposite. 

The client-side scanning solution is made worse by the opacity of mobile operating systems, which hinders any attempt to ensure that policies are  updated only by legitimate actors. Indeed, the opacity of the system as a whole hinders any attempt to ensure that the scanning capabilities are not used beyond law-enforcement needs.

We further show that the limitations of the technologies underlying client-side scanning cast extensive doubts about their effectiveness as monitoring tools. First, the limitations of automated recognition would unavoidably result in some information mistakenly reported as being targeted, undermining privacy for many users. Second, the poor performance of machine learning techniques in adversarial environments hints that scanning will both be easily evaded by criminals and will have high potential to be a new source of private information leaks due to the effectiveness of extraction attacks.

Finally, despite claims to the contrary, client-side scanning does not actually preserve confidentiality; it can offer, at best, ``selective confidentiality.'' The system allows end-to-end encryption of communication, but {\it only} after the communication has already been scanned for targeted content. Thus ``confidentiality'' is determined solely by the law-enforcement policy used to define what information is targeted. What is considered targeted, and may therefore leak, cannot be technically limited or controlled. In other words, client-side scanning can target any information, on any device, and thus readily be transformed into a mass surveillance infrastructure.

Our work builds on earlier efforts in this area. In particular, we show that client-side scanning fails to satisfy the Core Principles established in the recent {\it Moving the Encryption Policy Conversation Forward} from Carnegie Endowment for International Peace report\autocite{CEIP2019}. Client-side scanning is inherently non-transparent and not amenable to oversight. It cannot be limited in scope, the underlying techniques cannot be made specific and are prone to biases, and we cannot technically guarantee that only authorized parties can use the scanning capabilities. Client-side scanning is an opaque, uncontrollable intervention; its use would not just have a chilling effect on free speech, but is likely to create serious security risks to an infrastructure on which most of society now depends.

\section{Alternative Executive Summary by Jeff}

Public access to strong cryptography has been contentious since the mid-1970s. National-security forces tried to limit its use, then later law enforcement agencies pressed to do so. Many proposals have been suggested: key escrow and ``exceptional access'' mechanisms; none have found wide acceptance. Now some in industry and in government are advocating ``client-side scanning'' as a silver-bullet solution to the encryption quandary.

Client-side scanning is the examination of user content, writings, images, videos, speech on the user's device prior to encryption. This scanning will search for potentially illegal content and notify appropriate authorities when it is found.

It is hailed as a perfect solution that enables monitoring while leaving security and privacy intact. Instead of weakening encryption, or providing law enforcement with back doors.

Content, once scanned and determined to be legal, can be end-to-end encrypted as needed without compromising law enforcement's ability to monitor communications.

We show here that, contrary to the promise of an acceptable security trade-off, client-side scanning introduces serious risks to the security of ordinary users and to the information infrastructure as a whole.

It is worth noting that client-side scanning is not being proposed for use on targeted devices, such as those belonging to targets for which a warrant has been obtained, but instead on {\it everyone's} devices, lawbreakers and law-abiding citizens alike. It is mass surveillance, just automated and distributed.

Furthermore, such scanning is not without significant technical and operational issues:
\begin{itemize}
\item Automated scanning such as what will likely be used in client-side scanning is already in use privately by Cloud providers and Social Media providers. It frequently generates false-positive signals, the declaration that something inappropriate is happening, when in fact nothing untoward is happening.

\item The signals from scanning systems are often considered authoritative, requiring flagged individuals to prove their innocence, often after sanctions have already been applied. In the case of government sponsored client-side scanning, such sanctions may result in loss of freedom instead of just inconvenience.

\item Any deployed technology has the potential to be circumvented by bad actors. This may include subverting client-side technology to look for trade-secrets and report them to an adversary.

   [Note: for discussion later in the paper, all technology can be subverted, but client-side scanning provides just about all the capabilities that an attacker would want, minimizing the actual work they would have to perform to subvert a device with built-in client-side scanning.]
\end{itemize}

Finally, in a democratic nation, the ability of citizens to communicate freely depends strongly on their ability to feel safe in doing so. The specter of ``Big Brother'' always looking over your shoulder, which is what client-side scanning is, can provide a significant chilling effect on freedom of speech.


\section{Church quote}

To be used in text, perhaps in conclusions:

Indeed in 1976, the Church Committee of the U.S. Senate, investigating decades of surveillance abuses by the U.S. government, observed, 
\begin{quote}
  Persons most intimidated may well not be those at the extremes of the political spectrum, but rather those nearer the middle. Yet voices of moderation are vital to balance public debate and avoid polarization of our society.\autocite[p. 307]{United-States-Senate1976Intelligence-Ac}
  \end{quote}



\end{document}

